DRAGON: A Dialogue-Based Robot for Assistive Navigation with Visual Language Grounding

Persons with visual impairments (PwVI) have difficulties understanding and navigating spaces around them. Current wayfinding technologies either focus solely on navigation or provide limited communication about the environment. Motivated by recent advances in visual-language grounding and semantic navigation, we propose DRAGON, a guiding robot powered by a dialogue system and the ability to associate the environment with natural language. By understanding the commands from the user, DRAGON is able to guide the user to the desired landmarks on the map, describe the environment, and answer questions from visual observations. Through effective utilization of dialogue, the robot can ground the user's free-form descriptions to landmarks in the environment, and give the user semantic information through spoken language. We conduct a user study with blindfolded participants in an everyday indoor environment. Our results demonstrate that DRAGON is able to communicate with the user smoothly, provide a good guiding experience, and connect users with their surrounding environment in an intuitive manner. Videos and code are available at https://sites.google.com/view/dragon-wayfinding/home.

==> experiment.tex <==
\section{Experiments}
\label{sec::experiments}
LLfN is tested in simulated and physical experiments. We hypothesize that through LLfN (1) navigation performance can improve as the robot gathers more experience within a single environment, and (2) navigation in new environments can be learned while not forgetting how to navigate well in previous ones. 

\subsection{Robot Platform and Implementation}
\label{subsec::implementation}
Clearpath Jackal, a four-wheeled differential-drive unmanned ground vehicle, is used for both simulated and physical experiments. The robot is equipped with a laser scanner to perceive surrounding obstacles and runs the basic Robot Operating System (ROS) \texttt{move\textunderscore base} navigation stack. While the global planner is based on Dijkstra's algorithm \cite{dijkstra1959note}, the local planner uses DWA \cite{fox1997dynamic}, a sampling-based planner which may fail to sample feasible actions if not being properly tuned for the deployment environment. We fix the global planner and improve the local DWA planner using LLfN. We include the local goal provided by the global planner as part of the state, along with LiDAR input. Based on the local DWA planner as an initial policy ($\pi_0$), LLfN learns to complement this $\pi_0$ and improve navigation performance in multiple environments. When the sampling-based DWA cannot find feasible motion, it starts recovery behavior, including rotation in place or backing up \cite{zheng2017ros}. LLfN first improves navigation by eliminating those sub-optimal behaviors and producing alternative motions for a given environment. Second, it allows the robot to adapt to new environments while still remembering previous ones. 
% \peter{Have we introduced the notion of a global and local planner yet in this paper?  Does global appear in the algorithm?}

The learning problem is formulated as finding a policy $\pi_\theta$ that maps from the current state $s$, which includes LiDAR input (720- and 2095-dimensional for simulated and physical experiments, respectively) and local goal ($\left(x, y\right)$, 1m away on the global path), 
% \commentp{that's too informal a specification of the state space.  Be precise, give the dimensionality, etc.} 
to the action $a$, i.e. the linear velocity $v$ and angular velocity $\omega$.
In our implementation, the scoring function $D$ prioritizes actions proposed by DWA, if they result in a steady forward motion ($v\geq0.15\text{m/s}$, which is slightly larger than the minimal $v=0.1\text{m/s}$ to overcome friction). Importantly, all recovery behaviors from the DWA planner, including slowing down, turning in place, and moving backward, result in $v < 0.15\text{m/s}$. So with the above definition, $D$ will classify all recovery behaviors as suboptimal.
% This choice of implementation is due to the fact that DWA with default parameters is a relatively conservative algorithm, which only produces steady forward motion when it thinks the motion is absolutely safe.
Future works can investigate other implementations of $D$, or even learning it on the fly. If DWA fails to find feasible actions and would have started to execute recovery behaviors, the learned policy $\pi_\theta$ takes over. We acknowledge this implementation makes the scoring function $D$ not always accurate, e.g. it is possible that $D$ may prefer a bad action by $\pi_\theta$ when $\pi_0$ produces recovery behaviors. But in practice we observe LLfN remains effective even with such a simple $D$.

In consideration of limited onboard resources, we implement a streaming buffer $\mathcal{B}_\text{stream}$ as a regular queue to store 300 online streaming data points sequentially, and a separate memory $\mathcal{M}_\text{k}$ as a priority queue to save exemplar training data in the current environment. The number of data points within $\mathcal{B}\cup \{\mathcal{M}_k\}$ is also constrained to 300. The buffer sizes are empirically determined as the minimal value to assure efficient learning. For every sub-optimal action generated by DWA at a certain state, we compute a similarity score between this state and all states in the streaming buffer with a successful action (L2-norm of the LiDAR reading difference). We replace the data point of lowest similarity score in the training buffer with that from the streaming buffer.
% For duplicated entries, we simply update the similarity score.
% \peter{This detail also seems like it should have been introduced earlier.  The actually similarity score is an implementation detail.  But the way you get training data and trade off between the controller and the learned policy are aspects of the general algorithm, and should be introduced earlier.} \xuesu{see the comment above to add one more component}
The onboard data memory overhead to implement LLfN is \emph{at most} a total of 600 data points. 

\subsection{Simulated Experiments}
The effect of LLfN is first studied with extensive simulated trials. The simulated Jackal has a SICK LMS111 laser scanner onboard providing 270$^{\circ}$ 720-dimensional laser scan. The three simulated navigation environments are shown in Figure \ref{fig::sim_tasks}, where the robot navigates from a fixed start to a fixed goal in the environment. 
Env. 1's dense obstacles require fast response for obstacle avoidance; In Env. 2, the robot needs to keep a slow and consistent pace to drive through the narrow passage; Env. 3 requires the robot to slow down to make a sharp turn to enter the other room smoothly.

The robot is placed at its start location in each environment, and the learned policy $\pi_\theta$ to be tested is selected manually. 
\begin{figure}
\centering
\subfloat[Env. 1]{\includegraphics[height=1.33cm]{figures/Task1.jpg}%
\label{fig::task1}}
\hspace{2pt}
\subfloat[Env. 2]{\includegraphics[height=1.33cm]{figures/Task2.jpg}%
\label{fig::task2}}
\hspace{2pt}
\subfloat[Env. 3]{\includegraphics[height=1.33cm]{figures/Task3.jpg}%
\label{fig::task3}}
\caption{Simulated Navigation Environments: Green segments are primarily traversed using the initial policy $\pi_0$, while red segments are mostly traversed using the learned planner $\pi_\theta$. }
\label{fig::sim_tasks}
\vspace{-10pt}
\end{figure}
% \commentp{In the figure, it looks like the robot gets teleported from one environment to the next.  That's not the image I had from previous text and Figure 1 where it looks like there's some smooth transition from one environment to the next, but somehow the agent knows when it happens.  Also, remember you said the agent goes from one "end" of an environment to another, but that's not what it looks like in this figure.}

We use the initial policy $\pi_0$ to execute three trials in each of the three navigation environments to collect the training data. $\pi_0$ (DWA) can eventually navigate through, given sufficient time to recover, re-sample, and re-plan. 
% \commentp{This assumes that the initial policy can succeed at navigating through the whole environment, right?} 
To test in-environment learning improvement, training data of each given environment is \emph{divided into} 5 segments and incrementally presented to the learner. 
For example, the first training buffer for learning is constructed from the first one-fifth of the robot's experience, the second from the first two-fifths, etc. The last training buffer is from the entire experience. Note all these training buffers contain only 300 data points, who have the highest similarities to those states where the initial policy performs sub-optimally, given the presented navigation experience. 
% This results in training buffers of 300\peter{I don’t understand what you’re saying here.} data points with the highest similarities to those observations where the initial policy performs sub-optimally, given the presented navigation experience. 
Therefore, 6 incrementally learned navigation policies are produced, including the initial policy and the five policies learned from seeing 1/5, 2/5, ..., 5/5 of the training data from three training trials. Then the robot starts to learn the next navigation environment. For cross-environment learning, we use Sequential Training and the proposed LLfN. Sequential Training first uses the training buffer of environment 1. Starting with the final policy trained from environment 1, it sequentially trains on the training buffer of environment 2, before moving on to the training buffer of environment 3. In LLfN, while training environment 2, it only uses 150 data points from training buffer 2 with the highest similarity score, and still keeps a memory of 150 data points with the highest similarity score from training buffer 1 to assure new gradient updates won't increase the loss of environment 1. While training on environment 3, 100 data points with the highest similarity score for each environment are used, to avoid forgetting environment 1 and 2. 
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/sim_test.png}
\caption{Simulation Results: Each subplot (row $i$, column $j$) shows navigation performance with respect to increasing experience (x-axis), being trained using the $j$th and deployed in the $i$th environment. (Since there is no previous environment for Env. 1 and Train 1, both curves are the same.)}
\label{fig::sim_test}
\vspace{-10pt}
\end{figure}

We implement a small neural network of three hidden layers with 64 hidden neurons each, to compute linear and angular velocity based on the LiDAR input and local goal. After training, we evaluate the navigation performance in terms of traversal time in the current and previous environments. Each policy is executed three times, resulting in a total of 198 evaluation trials. We report the mean and standard deviation of the performance in Figure \ref{fig::sim_test}. If the robot is not able to reach the goal, e.g. gets stuck, a penalty time of 100s is given. Within each environment, LLfH is able to decrease traversal time with increasing learning experience. Across environments, LLfH learns new environments with increasing data while avoids catastrophic forgetting of previous ones. Sequential Training can improve navigation performance of a given environment when being presented the data from that particular environment, faster than LLfN. However, navigation performance in previous environments deteriorates with increasing experience in the current environment. The catastrophic forgetting is apparent in the diverging red line (Sequential Training) from the green line (LLfH). Note that the learned policies are used in conjunction with the initial policy in both cases. 

\subsection{Physical Experiments}
LLfN is also implemented on a physical Jackal robot. In the physical experiments (Figure \ref{fig::three_tasks}), we use the same setup, while all computation is done onboard the robot using an Intel Core i5-4570TE CPU. The physical Jackal has a Velodyne LiDAR, whose 3D point cloud data is converted to 360$^{\circ}$ 2095-dimensional laser scan. We design the physical test environments such that the goal of one environment smoothly transitions to the start of the next. Therefore the robot can traverse through all three environments in one shot. For training, we manually label the current environment for the learner. During deployment, the robot uses only one $\pi_\theta$ for each traversal. 

In the physical experiments, we compare LLfN with three baselines: DWA, Sequential Training, and Individual Models.
% \peter{That’s the right way to say it.  But then in Table 1, it again looks like GEM is what’s being compared.} 
Sequential Training and LLfN are conducted in the same way as in the simulated experiments. Individual Models are checkpoints of Sequentially Trained models up to the corresponding environment. Since these Individual Models do not suffer from forgetting, they serve as the \emph{best} models in Sequential Training. In contrast, the Sequentially Trained model is the final model after training on all 3 environments (thus ends up being much more effective on Environment 3 than Environment 1 or 2). The downside of Individual Models is that the number of models increases with the number of environments. Thanks to the constraint on data size, training each model takes less than two minutes on the robot's onboard CPU.
% \peter{The other thing that comes across to me gradually - really only in the experimental results section - is the fact that the default controller is used most of the time and the learned model is very sparsely used.  Presumably that’s why you can get away with so little data.  It’s a very specialized model.  I still find it confusing how much data is used to train the discriminator and the control policy, and exactly how they interact.  Actually, I’m now not sure that you have 2 different models.  I will go back and try figure it out.  But it needs to come out more clearly.  Another thing that could be useful to show is where along the trajectories in the environments the default controller and the learned policy are used.  How often is the policy invoked?  That would have to go in supplementary material, but at least in simulation, is it possible to illustrate?}
% \begin{wraptable}{r}{0.6\textwidth}
\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{cccccc}
\toprule
& & \textbf{DWA} & \textbf{\begin{tabular}[c]{@{}c@{}}Sequential \\ Training\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLfN\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Individual\\ Models\end{tabular}} \\ \midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Env. 1}}} & Time & 38.36$\pm$1.69  & 39.11$\pm$6.45 & \textbf{28.32}$\pm$1.85  & 30.17$\pm$\textbf{0.97}\\ 
\multicolumn{1}{c}{} & Rec./Col. & 1.8/0 & 1.4/0.6 & 0/0 & 0/0\\ \midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Env. 2}}} & Time               & 28.05$\pm$3.48 & 49.41$\pm$ 13.94 & \textbf{19.98}$\pm$1.07 & 23.41$\pm$\textbf{0.66}\\
\multicolumn{1}{c}{} & Rec./Col. & 1.4/0.2 & 1.25/0.8 & 0/0 & 0/0 \\ \midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Env. 3}}} & Time & 39.80$\pm$6.39  & 21.12$\pm$1.17 & 21.80$\pm$1.51 & \textbf{21.12}$\pm$\textbf{1.17} \\ 
\multicolumn{1}{c}{} & Rec./Col. & 2.2/0.2 & 0/0 & 0/0 & 0/0\\ \bottomrule
\end{tabular}}
\caption{~Physical Results after Training on 3 Environments: Time (in s), Number of Recovery Behaviors (Rec.) and Collisions (Col.).}
\vspace{-5pt}
\label{tab::experiments}
\end{table}
We deploy the trained models to navigate in the three environments. For each method, the robot navigates each environment five times, resulting in a total of 60 physical trials. Table \ref{tab::experiments} reports the mean execution time for each environment with standard deviation and average number of recovery behaviors (Rec.) and collisions (Col.). 
DWA exhibits the most recovery behaviors, because whenever the robot fails to sample a feasible motion, it starts recovery behavior. One collision happens in one of the environment 2 and 3 trials. Applying the model sequentially learned on environment 1, 2, and 3 causes catastrophic forgetting of the first two environments. It leads to longer execution time and higher standard deviation, with frequent recovery behaviors and collisions. LLfN can successfully avoid catastrophic forgetting: It achieves a similar time to the Individual Models approach in environment 3, while, \emph{surprisingly}, it outperforms Individual Models in environment 1 and 2 in terms of average time. One possible explanation is that the LLfN model has good backward transfer ability after gathering more diverse experience.
Utilizing extra training data and models specifically trained for each environment, the Individual Models approach is more stable (lowest standard deviation). (Video of representative trials of the four methods: \url{www.youtube.com/watch?v=ja_Rjc63xiY&t=68s}.)


